Multiplicities and dimensions in enveloping tensor categories

In the previous paper arxiv:math/0610552 semisimple tensor categories were constructed out of certain regular Mal'cev categories. In this paper, we calculate the tensor product multiplicities and the categorical dimensions of the simple objects. This yields also the Grothendieck ring. The main tool is the subquotient decomposition of the basic objects.

==> amsart-modif.tex <==
\catcode`\@=11

%Changes \title@amsart: flush left instead of uppercase centered

\def\@settitle{%
  \baselineskip14\p@\relax
    {\Large\bfseries%\fontsize{24}{18}\selectfont%
  \@title}}

%Changes author@amsart: Small caps flush left instead of uppercase centered

\def\@setauthors{%
  \begingroup
  \def\thanks{\protect\thanks@warning}%
  \trivlist
  \footnotesize \@topsep45\p@\relax
  \advance\@topsep by -\baselineskip
  \item\relax
  \author@andify\authors
  \def\\{\protect\linebreak}%
  {\sc\fontsize{12}{10}\selectfont\authors}%
  \ifx\@empty\contribs
  \else
    ,\penalty-3 \space \@setcontribs
    \@closetoccontribs
  \fi
  \endtrivlist
  \endgroup
}

%Changes section@amsart: Bold flush left instead of small caps centered

\def\@secnumfont{\bfseries}%

\def\section{\@startsection{section}{1}%
  \z@{.7\linespacing\@plus\linespacing}{.5\linespacing}%
  {\normalfont\bf}}

%Changes citation labels@amsrefs: flush left instead of flush right

% \renewcommand{\BibLabel}{%
% %    \hfill
%     \Hy@raisedlink{\hyper@anchorstart{cite.\CurrentBib}\hyper@anchorend}%
%     [\thebib]\hfill%
% }
% \BibLabel=\long macro:
% ->\hfill \Hy@raisedlink {\hyper@anchorstart {cite.\CurrentBib }\hyper@anchorend }[\thebib ]

%New label "arxiv"

\DefineSimpleKey{bib}{arxiv}

% \BibSpec{article}{%
%     +{}  {\PrintAuthors}                {author}
%     +{,} { \textit}                     {title}
%     +{.} { }                            {part}
%     +{:} { \textit}                     {subtitle}
%     +{,} { \PrintContributions}         {contribution}
%     +{.} { \PrintPartials}              {partial}
%     +{,} { }                            {journal}
%     +{}  { \textbf}                     {volume}
%     +{}  { \PrintDatePV}                {date}
% %    +{,} { \issuetext}                  {number}
%     +{,} { \eprintpages}                {pages}
%     +{,} { }                            {status}
% %    +{,} { \PrintDOI}                   {doi}
% %    +{}  { \parenthesize}               {language}
%     +{}  { \PrintTranslation}           {translation}
%     +{;} { \PrintReprint}               {reprint}
%     +{.} { }                            {note}
%     +{.} {}                             {transition}
% %    +{}  {\SentenceSpace \PrintReviews} {review}
%     +{,} { \arxiv}           {arxiv}
%   }

\BibSpec{article}{%
    +{}  {\PrintAuthors}                {author}
    +{,} { \textit}                     {title}
    +{.} { }                            {part}
    +{:} { \textit}                     {subtitle}
    +{,} { \PrintContributions}         {contribution}
    +{.} { \PrintPartials}              {partial}
    +{,} { }                            {journal}
    +{}  { \textbf}                     {volume}
    +{}  { \PrintDatePV}                {date}
%    +{,} { \issuetext}                  {number}
    +{,} { \eprintpages}                {pages}
    +{,} { }                            {status}
%    +{,} { \PrintDOI}                   {doi}
%    +{}  { \parenthesize}               {language}
    +{}  { \PrintTranslation}           {translation}
    +{;} { \PrintReprint}               {reprint}
    +{.} { }                            {note}
    +{,} { \arxiv}           {arxiv}
    +{.} {}                             {transition}
%    +{}  {\SentenceSpace \PrintReviews} {review}
  }

\BibSpec{collection.article}{%
    +{}  {\PrintAuthors}                {author}
    +{,} { \textit}                     {title}
    +{.} { }                            {part}
    +{:} { \textit}                     {subtitle}
    +{,} { \PrintContributions}         {contribution}
    +{,} { \PrintConference}            {conference}
    +{}  {\PrintBook}                   {book}
    +{,} { }                            {booktitle}
    +{} { \PrintDate}                  {date}
    +{,} { }                        {pages}
    +{,} { }                            {status}
    +{,} { \PrintDOI}                   {doi}
    +{,} { available at \eprint}        {eprint}
    +{,} { \arxiv}           {arxiv}
%    +{}  { \parenthesize}               {language}
    +{}  { \PrintTranslation}           {translation}
    +{;} { \PrintReprint}               {reprint}
    +{.} { }                            {note}
    +{.} {}                             {transition}
%    +{}  {\SentenceSpace \PrintReviews} {review}
}

\BibSpec{book}{%
    +{}  {\PrintPrimary}                {transition}
    +{,} { \textit}                     {title}
    +{.} { }                            {part}
    +{:} { \textit}                     {subtitle}
    +{,} { \PrintEdition}               {edition}
    +{}  { \PrintEditorsB}              {editor}
    +{,} { \PrintTranslatorsC}          {translator}
    +{,} { \PrintContributions}         {contribution}
    +{,} { }                            {series}
    +{,} { \voltext}                    {volume}
    +{,} { }                            {publisher}
    +{,} { }                            {organization}
    +{,} { }                            {address}
    +{} { \PrintDate}                 {date}
    +{,} { }                            {status}
    +{}  { \parenthesize}               {language}
    +{}  { \PrintTranslation}           {translation}
    +{;} { \PrintReprint}               {reprint}
    +{.} { }                            {note}
    +{.} {}                             {transition}
%    +{}  {\SentenceSpace \PrintReviews} {review}
}


%\newcommand{\arxiv}[1]{\href{http://arxiv.org/abs/#1}{{\tt arxiv:\hspace{0pt}#1}}}
\newcommand{\arxiv}[1]{\tt arxiv:\hspace{0pt}{\href{http://arxiv.org/abs/#1}{#1}}}

\renewcommand{\voltext}{\IfEmptyBibField{series}{\textbf}{\textbf}}

\renewcommand{\BibLabel}{%
    \Hy@raisedlink{\hyper@anchorstart{cite.\CurrentBib}\hyper@anchorend}%
    [\thebib]}

\catcode`\@=12
